GEAR-RT: Towards Exa-Scale Moment Based Radiative Transfer For Cosmological Simulations Using Task-Based Parallelism And Dynamic Sub-Cycling with SWIFT

The development and implementation of GEAR-RT, a radiative transfer solver using the M1 closure in the open source code SWIFT, is presented, and validated using standard tests for radiative transfer. GEAR-RT is modeled after RAMSES-RT (Rosdahl et al. 2013) with some key differences. Firstly, while RAMSES-RT uses Finite Volume methods and an Adaptive Mesh Refinement (AMR) strategy, GEAR-RT employs particles as discretization elements and solves the equations using a Finite Volume Particle Method (FVPM). Secondly, GEAR-RT makes use of the task-based parallelization strategy of SWIFT, which allows for optimized load balancing, increased cache efficiency, asynchronous communications, and a domain decomposition based on work rather than on data. GEAR-RT is able to perform sub-cycles of radiative transfer steps w.r.t. a single hydrodynamics step. Radiation requires much smaller time step sizes than hydrodynamics, and sub-cycling permits calculations which are not strictly necessary to be skipped. Indeed, in a test case with gravity, hydrodynamics, and radiative transfer, the sub-cycling is able to reduce the runtime of a simulation by over 90%. Allowing only a part of the involved physics to be sub-cycled is a contrived matter when task-based parallelism is involved, and is an entirely novel feature in SWIFT. Since GEAR-RT uses a FVPM, a detailed introduction into Finite Volume methods and Finite Volume Particle Methods is presented. In astrophysical literature, two FVPM methods are written about: Hopkins (2015) have implemented one in their GIZMO code, while the one mentioned in Ivanova et al. (2013) isn't used to date. In this work, I test an implementation of the Ivanova et al. (2013) version, and conclude that in its current form, it is not suitable for use with particles which are co-moving with the fluid, which in turn is an essential feature for cosmological simulations.

==> tables/ACACIA/observed_smfs.tex <==
\begin{table}
	\centering
	\caption{
		Redshift interval of observed stellar mass functions that are used for comparison and the abbreviation used in this work as reference.
		}
	\label{tab:obs_smf}
	\begin{tabular}[c]{l l l}
			redshifts		        & Reference						& 	Abbreviation \\
		\hline
			$z \sim 0 - 1 $			& \cite{OBS_moustakas}			& 	MOU	\\				
%
			$z \sim 0 - 4 $			& \cite{OBS_perez-gonzalez}		& 	PG \\			
%
			$z \sim 1 - 3.5 $		& \cite{OBS_mortlock}			& 	MOR	\\
%
			$z \sim 1.3 - 4.0$		& \cite{OBS_marchesini}			&   MAR  \\
%
%			$z \sim 4$, $z \sim 5$	& \cite{OBS_kslee}				& 	KSL	\\
%%
%			$z \sim 4 - 6 $			& \cite{OBS_stark}				& 	ST	\\
%%	
%			$z \sim 7$, $z \sim 8$	& \cite{OBS_bouwens}			&	BOU	\\
	\end{tabular}
\end{table}
